ALBUS: a Probabilistic Monitoring Algorithm to Counter Burst-Flood Attacks

Modern DDoS defense systems rely on probabilistic monitoring algorithms to identify flows that exceed a volume threshold and should thus be penalized. Commonly, classic sketch algorithms are considered sufficiently accurate for usage in DDoS defense. However, as we show in this paper, these algorithms achieve poor detection accuracy under burst-flood attacks, i.e., volumetric DDoS attacks composed of a swarm of medium-rate sub-second traffic bursts. Under this challenging attack pattern, traditional sketch algorithms can only detect a high share of the attack bursts by incurring a large number of false positives. In this paper, we present ALBUS, a probabilistic monitoring algorithm that overcomes the inherent limitations of previous schemes: ALBUS is highly effective at detecting large bursts while reporting no legitimate flows, and therefore improves on prior work regarding both recall and precision. Besides improving accuracy, ALBUS scales to high traffic rates, which we demonstrate with an FPGA implementation, and is suitable for programmable switches, which we showcase with a P4 implementation.

==> makefile <==
FILES = main
# FILES = $(patsubst %.tex,%,$(wildcard *.tex))
FILES_PDF = $(addsuffix .pdf,$(FILES))
FILES_FINAL_PDF = $(addsuffix -final.pdf,$(FILES))
FILES_DIFF_PDF = $(addsuffix -diff.pdf,$(FILES))

.PHONY: $(FILES_PDF) $(FILES_FINAL_PDF) $(FILES_DIFF_PDF) all clean final diff.pdf

all: $(FILES_PDF) $(FILES_FINAL_PDF)

final: $(FILES_FINAL_PDF)

$(FILES_PDF): %.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape $<

$(FILES_FINAL_PDF): %-final.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape -pdflatex='pdflatex %O -interaction=nonstopmode -synctex=1 "\newcommand{\final}{}\input{%S}"' $<


P = paper

# default : $P.pdf

# $P.dvi	: $(wildcard *.tex *.bib figures/*.eps)
# 	latex  $P < /dev/null || $(RM) $@
# 	bibtex $P < /dev/null || $(RM) $@
# 	latex  $P < /dev/null || $(RM) $@
# 	latex  $P < /dev/null || $(RM) $@

# $P.pdf  : $(wildcard *.tex *.bib figures/*)
# 	pdflatex --shell-escape $P
# 	bibtex $P
# 	pdflatex --shell-escape $P
# 	pdflatex --shell-escape $P

# $P.ps	: $P.dvi
# 	dvips -tletter -Ppdf $P.dvi -o $P.ps

# $P.ps.gz: $P.ps
# 	$(RM) $P.ps.gz
# 	gzip -9 < $P.ps > $P.ps.gz

# print:	$P.ps

# dist:	$P.ps.gz

clean:
	$(RM) *.log *.aux *.bbl *.blg *.out *.dvi *.ps *.ps.gz *.fdb_latexmk *.synctex.gz *.fls texput.log


==> sec/algorithm-code.tex <==
\appendix

\section{Pseudocode of \name{}}
\label{sec:appendix:pseudocode}

\Cref{alg:our-algo} contains a 
pseudocode representation of the
\name{} algorithm.

\begin{algorithm}
\caption{\name{}}\label{alg:our-algo}
\begin{algorithmic}
\Function{Update}{Flow ID $f$, packet size~$s$, timestamp~$t$}
\State $i \gets \mathit{hash}(f)$
\quad $\lambda \gets \Lambda[i]$
\quad $\pi \gets \Pi[i]$
\If{$\lambda.f = f$}  \Comment{Update leaky bucket}
\State $d \gets \gamma \cdot (t - \lambda.t)$
\State $\lambda.c \gets \max(\lambda.c - d, 0) + s$
\If{$\lambda.c > \beta$} \Comment{Found excessively bursty flow}
    \State $\lambda.f \gets \pi.f$
    \quad $\lambda.t \gets -\infty$\
    \quad $\lambda.c \gets 0$
    \State $\pi.f \gets \bot$
    \quad $\pi.c \gets 0$
    \State \Return \text{True}
\ElsIf{$s < d$} \Comment{Replace non-bursty flow}
    \State $\lambda.f \gets \pi.f$
    \quad $\lambda.t \gets -\infty$
    \quad $\lambda.c \gets 0$
    \State $\pi.f \gets \bot$
    \quad $\pi.c \gets 0$
\EndIf
\State \Return \text{False}
\ElsIf{$\lambda.f = \bot$} \Comment{Fill unassigned leaky bucket}
    \State $\lambda.f \gets f$
    \quad $\lambda.t \gets t$
    \quad $\lambda.c \gets 0$
    \State \Return \text{False}
\ElsIf{$\lambda.t < t-\frac{\beta}{\gamma}$} \Comment{Check time-out}
    \State $\lambda.f \gets \pi.f$
    \quad $\lambda.t \gets -\infty$
    \quad $\lambda.c \gets 0$
    \State $\pi.f \gets \bot$
    \quad $\pi.c \gets 0$
    \State \Return \text{False}
\EndIf
\If{$\pi.f = f$}  \Comment{Update PF counter}
    \State $\pi.c \gets \pi.c + s$
    \If{$\pi.c > T$} \Comment{Masking-attack safeguard}
        \State $f' \gets \lambda.f$ 
        \quad $c' \gets \lambda.c$ 
        \State $\lambda.f \gets f$
        \quad $\lambda.t \gets t$
        \quad $\lambda.c \gets 0$
        \State $\pi.f \gets f'$
        \quad $\pi.c \gets c'$
    \EndIf
\ElsIf{$\pi.f = \bot$} \Comment{Fill unassigned PF counter}
    \State $\pi.f \gets f$
    \quad $\pi.c \gets s$
\ElsIf{$x \sim \mathcal{U}_{[0,1]} < 0.1^r$} \Comment{Probabilistic decay}
    \If{$s > \pi.c$}
        \State $\pi.f \gets f$ 
        \quad $\pi.c \gets s$
    \Else{} 
        \State $\pi.c \gets \pi.c - s$
    \EndIf
\EndIf
\State \Return \text{False}
\EndFunction
\end{algorithmic}
\end{algorithm}



